Learn Like The Pro: Norms from Theory to Size Neural Computation

The optimal design of neural networks is a critical problem in many applications. Here, we investigate how dynamical systems with polynomial nonlinearities can inform the design of neural systems that seek to emulate them. We propose a Learnability metric and its associated features to quantify the near-equilibrium behavior of learning dynamics. Equating the Learnability of neural systems with equivalent parameter estimation metric of the reference system establishes bounds on network structure. In this way, norms from theory provide a good first guess for neural structure, which may then further adapt with data. The proposed approach neither requires training nor training data. It reveals exact sizing for a class of neural networks with multiplicative nodes that mimic continuous- or discrete-time polynomial dynamics. It also provides relatively tight lower size bounds for classical feed-forward networks that is consistent with simulated assessments.

==> tex/foo.tex <==
To extend the methodology to discrete-time networks, consider for the purpose of this version of this paper, the class of of autonomous equations $\dot{x} = f_{NN}(x)$, with $x_0= x(0)$. We further consider two common classes of ode solvers, which are  expressed as neuro-logic networks.

\begin{figure}[ht]
\centering
\includegraphics[width=0.9\linewidth]{figures/abm2.png}
\caption{Adams-Bashforth Predictor coupled with an Adams-Moulton Corrector. }
\label{fig:ab2}
\end{figure}

Consider a two-step Adams-Bashforth predictor, coupled to a two-step Adams-Moulton the corrector, such as: 
\begin{eqnarray}
\label{eq:ab2}
P_{n+1}&=&x_{n}+{\frac {3}{2}}hf_{NN}(x_{n})-{\frac {1}{2}}hf_{NN}(x_{n-1})\\
    x_{n+1}&=&x_{n}+{\tfrac {1}{2}}h\left(f_{NN}(P_{n+1})+f_{NN}(x_{n})\right)
\end{eqnarray}

\begin{figure}[ht]
\centering
%\includegraphics[width=0.9\linewidth]{figures/rk45net.png}
\includegraphics[width=0.95\linewidth]{figures/NEURK4.png}
\caption{A neural circuit for an explicit fourth-order Runge Kutta method. }
\label{fig:rk4}
\end{figure}

Further consider a fourth-order Runge-Kutta method
\begin{eqnarray}
 k_1 &=& h f_{NN}(x_n)\\
 k_2 &=& h f_{NN}(x_n+\frac{1}{2} k_1) \\
 k_3 &=& h f_{NN}(x_n + \frac{1}{2} k_2) \\
 k_4  &=& h f_{NN}(x_n + k_3) \\
 x_{n+1} &=& x_n + \frac{1}{6} (k_1 + 2\;k_2+ 2\;k_3 + k_4)
\end{eqnarray}
 The neural circuit in Figure~\ref{fig:ab2} implements, in recurrent form, the predictor corrector method. It has an input node (purple), hidden nodes (gray)  and an output node (orange), all of which are additive with linear activation. Edges are explicitly labeled with weights, otherwise they are $1$. Feedbacks in the recurrence are delayed one discrete step.  When input $x_n$ arrives, the recurrent state is holding $-\frac{h}{2}f_{NN}(x_{n-1})$ and the flow of computation implements Equations~\ref{eq:ab2}. The output is returned to the stream and becomes the input at the next time step when the recurrent state is holding $-\frac{h}{2}f_{NN}(x_{n})$. The network in Figure~\ref{fig:ab2} can be appended to the continuous time network in Figure~\ref{fig:lornet} to produce a complete discrete-time network neural simulator that is by construction identical to the similarly implemented numerical model. 
 
 Figure~\ref{fig:rk4} depicts a circuit with linearly activated summation nodes (blue) interspersed with the neural subroutine that calculates the continuous rates of change. As with the parameterization argument, if the step $h$ is held fixed, then the number of free parameters to match learnability doesn't change.  For the Lorenz system, this implies they are simply a class of neural networks. In this way, theory describing polynomial nonlinear dynamics can be used to directly synthesize optimal networks identical to their numerical counterparts. Several other examples are illustrated in Part II of this work.
 
 The solutions of the Lorenz model are known to be dissipative (volume in phase contracts rapidly), and chaotic (sensitive to initial perturbations). Despite being derived from a physical system, the ad-hoc truncations make L63 deviate from the RB convection \textcolor{blue}{\cite{Curry1978, Berge1987}} and  therefore it is only used as a simplified chaotic dynamical model for our purpose. 

L63 can also be defined as a discrete mapping that maps the current state of the system $\mathbf{x}_n = (X, Y, Z)^{\mathrm{T}}$ to the state of the next timestep $\mathbf{x}_{n + 1}$: 
\begin{equation}
\begin{aligned}
&\Phi_{\mathrm{L63}}(\mathbf{x}_n) =  \mathbf{x}_{n + 1}.
%&\Phi_{\mathrm{L63}} : \mathbb{R}^3 \mapsto \mathbb{R}^3 : \mathbf{x}_n \mapsto \mathbf{x}_{n + 1}. 
\label{eq:mapping_discrete}
\end{aligned}
\end{equation}
%Although L63 was originally defined in the differential fashion, 
This discrete form is chosen in this paper both for the L63 and NN because it provides a deeper connection between the geometric L63 mapping and the structure of the neural network. In practice, since the exact form of equation (\textcolor{red}{\ref{eq:mapping_discrete}}) for L63 is unknown, the mapping is obtained by numerically integrate equation (\textcolor{red}{\ref{eq:L63}}) in time with a discrete increment $\mathrm{d}t$. 

The discrete mapping implemented by a single-hidden-layer feedforward NN is 
%$\mathbf{x}_{n+1} = \Phi_{\mathrm{NN}}(\mathbf{x}_n) = \mathbf{W_2}g(\mathbf{W_1}\mathbf{x}_n + \mathbf{b_1}) + \mathbf{b_2}$.
\begin{equation}
\Phi_{\mathrm{NN}}(\mathbf{x}_n) = \mathbf{W_2}g(\mathbf{W_1}\mathbf{x}_n + \mathbf{b_1}) + \mathbf{b_2}, 
\label{eq:NN}
\end{equation}
in which the $3\times1$ input vector $\mathbf{x}_{n}$ is first multiplied by an $L\times3$ weight matrix $\mathbf{W_1}$ from the left, and added to an $L\times1$ bias term $\mathbf{b_1}$, where $L$ is the number of neurons. The resulting $L\times1$ vector is then element-wise ``compressed" by a sigmoid function $g(\cdot)$, which takes the form of $\tanh$ in our setup.  Multiplication by a $3\times L$ matrix $\mathbf{W_2}$ from the left followed by addition of another bias term $\mathbf{b_2}$ finishes a mapping iteration of the NN. 

We use Matlab function \textit{ode45} to numerically solve for the discrete mappings of L63 as training data. To obtain data on the attractor, we initialize 1000 trajectories whose initial points are uniformly sampled from region $\{x\in[-20, 20],y\in[-20, 20],z\in[0, 50]\}$. Each trajectory is integrated for 2500 timesteps with increment $\mathrm{d}t = 0.01$. The first 2000 timesteps are abandoned so that the transient parts of the trajectories (much shorter than 2000 steps) are omitted. Then, the remaining 500 timesteps of the 1000 trajectories are aggregated as pairs $(\mathbf{x}, \mathbf{x'})$ that satisfy $\mathbf{x'} = \Phi_{L63}(\mathbf{x})$, forming the training data pool. 
%The positions of these points are also a representation of the L63 attractor. 
The NN is trained for $10^3$ epochs with Bayesian regularization \textcolor{blue}{\cite{DanForesee1997}}. 



\textit{Results} -- We first quantify how well NN can learn the chaotic dynamics of L63 with a small amount of data and neurons. The quadratic prediction error is reported elsewhere \textcolor{blue}{\cite{Zhang2017b}}, and will not be the main focus of this paper. 

NN can also extrapolate well from an incomplete training dataset. Figure \textcolor{red}{\ref{fig:NN_predictions}} shows a comparison of two trajectories predicted by NN and L63 that originate from the same position. The NN in this case has 5 neurons, and is trained on 100 data points sampled from the $X>-5$ region of attractor $\mathcal{A}_{\mathrm{L63}}$, which amounts to knowing 73\% of the attractor structure. The two trajectories are close in the first 100 timesteps, and then bifurcate onto the two branches of the attractor. Despite starting from an unknown region, the NN still predicts a well-behaved structure that closely resembles the original attractor in the extrapolated region of $X\le-5$. Moreover, the FTLEs of NNs with different complexities trained on incomplete data of this fashion have a one-to-one correspondence similar to figure \textcolor{red}{\ref{fig:FTLE}} (not shown).  
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/NN_predictions_3D_half_domain.png}
\caption{Two trajectories produced by L63 (blue) and a 5-neuron NN trained on 100 data points sampled from $X>-5$ (red). The region to the right of the grey partition is the training data range, and the region to the left is unknown to the NN. }
\label{fig:NN_predictions}
\end{figure}
 
 \subsection{Spectral Norm and Learnability Number}
Similar analysis may be performed approaching convergence during learning. Away from equilibrium, the error may be factorized as $e_{is} = \bar{e}_i+\tilde{e}_s$, for some weights $w_i$ and $\sum_s \tilde{e}_s =0$. Now consider the variational problem for a small perturbation from the unknown equilibrium $w_0 = w_* + \delta w$ and the least squares objective over a batch of data $S$:
\begin{equation}
    J(w):= \frac{1}{2S}\sum_{s=1}^S (y_s - f(x_s; w))^2
\end{equation}
Further consider the nominal gradient descent rule:
\begin{eqnarray}
    w_{i+1} &=& w_i - \alpha \frac{\partial J}{\partial w_i}
\end{eqnarray}
solved iteratively with initial condition $w_0$, that upon convergence $w_M, M>0$ is an estimate of $w_*$. The gradient may be further expanded at iteration $i$ as
\begin{eqnarray}
        w_{i+1}&=& w_i + \frac{\alpha}{S}  \sum_{s=1}^S  \nabla_{w_i} f(x_s;w_i)^T e_{is}
\end{eqnarray}
We model $\nabla_{w_i} f(x_s;w_i) = \bar{F}_i +\tilde{F}_s$ with $\sum_s \tilde{F}_s = 0$ and assume the errors and parameters (gradients) are independent near equilibrium, so that $\sum_s  \tilde{F}_s^T \tilde{e}_s= 0$. With these assumptions, we may express the update as: 
\begin{eqnarray}
    w_{i+1} &=& w_i + \alpha  \bar{F}_i^T \bar{e}_{i}
    \label{eq:gradient}
\end{eqnarray}
Consequently, we may write the error growth/decay as
\begin{eqnarray}
    e_{i+1,s} &=& y_s-f(x_s;w_i + \alpha  \bar{F}_i^T \bar{e}_{i})
\end{eqnarray}
Which, via a first order Taylor expansion yields
\begin{equation}
    U^T_i \delta  \bar{e}_{i} = -\alpha\Sigma^2_i U_i^T\bar{e}_{i}
\end{equation}
where $\delta  \bar{e}_{i} = [\bar{e}_{i+1} - \bar{e}_i]$ and $G_i=\bar{F}_i \bar{F}^T_i$, and the eigenvalue decomposition $G_i U_i = U_i\Sigma^2_i$ for the diagonal eigenvalue matrix $\Sigma_i$ and unitary transform $U_i$. Thus, we may write a bound
\begin{equation}
\label{eq:derdesc}
    |\delta  \epsilon_i|  \leq \alpha\sigma^2_{m,i} |\epsilon_i|
\end{equation}
where $\epsilon_i = \pm \sqrt{\bar{e}_{i}^T\bar{e}_{i}}$ and $\delta \epsilon = \pm \sqrt{(\delta\bar{e}_{i})^T \delta\bar{e}_{i}}$. Further, 
\begin{eqnarray}
U^T_i \bar{e}_{i+1} &=& [I-\alpha\Sigma^2_i] U_i^T\bar{e}_{i}\\
\label{eq:desc}\Rightarrow\epsilon_{i+1}^2 & \leq & (1-\alpha\sigma^2_{m,i})^2 \epsilon_i^2
\end{eqnarray}


  From Equation~\ref{eq:desc} and Equation~\ref{eq:derdesc}, not that gain $0<\alpha\sigma^2_{m,i}<1$ establishes a converging sequence. This is related to the local Lyapunov number of the dynamical system\textcolor{blue}{\cite{Haller2001}} that learning implies, and it naturally also relates to stability. Following the Learnability metric, here, we call $\sigma^2_{m,i}$ the local {\em leading Learnability} number. Two systems may be related by comparing their Learnability numbers. 
  That is, the parameter-Jacobian of the polynomial dynamical system $F_{poly}$ has a Frobenius norm ($||\cdot||_{fr}^2$) that is the trace of the Learnability metric (equivalently its eigen values). We call this the {\it total Learnability number}. It is invariant to all unitary transformations of $G_{poly}$, the induced metric. 

bounds the error 2-norm: 
A straightforward interpretation  is that the Frobenius norm of $F_s$ controls the magnitude of error reduction (increase) as one moves toward (away from)  learning equilibrium. 

Where, the eigenvalue decomposition is. The matrix $G:=<G_s>$ is the expected Frobenius norm of the parameter Jacobian over the batch (or mini-batch), whose  gradients prescribe preferred directions for learning. To see this, note that 




 Learnability metrics allow comparisons between systems with arbitrarily different parameter spaces. For example, a polynomial learning system and a neural learning system under unit norm perturbation of their respective parameters yields the equivalence: 
\begin{eqnarray}
\label{eq:frob}
%\frac{tr(\Sigma_s^2_{nn})}{\epsilon^2_{nn}} & =& c \frac{tr(\Sigma^2_{poly})}{\epsilon^2_{poly}}\\
{tr(\Sigma^2_{nn})} & =& c\eta^2 \; {tr(\Sigma^2_{poly})} 
\end{eqnarray}
 where, $c$ is a constant, $\eta = \frac{|\epsilon_{nn}|}{|\epsilon_{poly}|}$ is a relative efficacy. If this is specified, then the Learnability metrics, which are equivalent to the Frobenious norms of their parameter Jacobians, allow us to compare their learning behavior. As we shall see, if Learnability can be parameterized by size parameters (e.g. network size), then we might be able to estimate it by equating it to another ``known'' system.

We define two systems with a common learning rate and spetcral/Frobenius norm as equivalent learners. Thus, if one were to consider a polynomial system and the other a neural network, then comparing the norms of spectra as discussed in the previous section establishes a functional equivalence of how the two learn. Such functional equivalence does not guarantee by itself that either system will learn a mapping. However, one can say that  one is ``as good as" the other. 


In the unrestricted PolyNet, there are $n^2$ direct connections between inputs and outputs $n$ output bias terms, $L$ hidden bias terms, and $nL$ weight input-hidden, hidden-output weight terms. Subclasses that remove certain terms (e.g. biases) can be derived from this network easily. As before the activations are pass-through, multiplicative or additive nodes may be included as 
We model the L63 with an $n=3$ and $d=2$ polynomial, arbitratily set $\eta = 1$ and $c=1$. This implies that  at least two hidden nodes would be needed. Is this feasible? Under what type of activation? The only demands we make is that suitable scaled, the leading Lyapunov number is bounded by $2nL$. Figure~\ref{fig:lornet} shows that this is in fact trivial and the construction is exact. There is a neural network with multiplicative nodes that operates in continuous-time, meaning it predicts $\dot{x}, \dot{y}, \dot{z}$ instead of a discrete map obtained by discretizing the governing equations. Such a neural system must still be integrated, for which traditional $ODE$ solvers may be used. 



Consider all bounded inputs in the unit $n$-dimensional hypercube and consider random weights in the interval $[-1, 1]$\footnote{These input and weight systems are not restrictive; a single normalization is needed for reduction from other systems.}. The Frobenius norm (squared) is bound by $O(n^2L)$.


Consider the second polynomial system of maximum degree $d$ and inputs of length $n$ and bounded in the same manner.  The polynomial has ${n+d \choose d}$ monomials, thus its Spectral norm is bound by $O({n+d \choose d})$ and the Frobenius norm by $O(n{n+d \choose d})$. Therefore, matching the bounds provides a nominal constraint: 
\begin{equation}
\label{eq:hidden}
   L = O\left( \frac{\eta^2}{n} {{n+d \choose d} }\right)
\end{equation}

Where $\eta = \frac{|\epsilon_{nn}|}{|\epsilon_{poly,\infty}|}\geq 1$ is a desired relative efficiency. This follows from Equation~\ref{eq:frob}. As we shall shortly see, the nominal constraint can be further tightened.

\subsection{Exact Poly-Nets}

If neural networks admitted multiplicative nodes~\cite{trautner19}, which has been suggested as a pathway to model polynomials~\cite{Andoni2014}, then dynamical systems with polynomial nonlinearities have trivial exact neural networks called PolyNets~\cite{trautner19}. 

have been shown to exactly model continuous polynomial dyanm a $n$ input polynomial with maximum degree $d$. Given our interest in autonomous dynamical systems with polynomial non-linearities in this paper, consider a polynomyial system of the form $dot{x} = f(x_t;\alpha)$, $x_t\in\Re^n$. The parameters are  $m = {n+d \choose d}$ with $\alpha\in \Re^m$. We divide the parameter vector further as $\alpha = \{\alpha_{i,k}\}, i=1\ldots n, k=0\ldots m-1$, where we reserve $\alpha_{i,0}$ for the degree $d=0$ parameters $\alpha_{i,1\ldots n}$ for the degree $d=1$ parameters.

Define the neural network $y=f_{NN}(x)$ with $x,y\in \Re^n$ being the inputs and outputs respectively, and one hidden layer with $h=max\left(0,n\times\left( {n+d \choose d}-n - 1\right)\right)$ nodes, $z \in \Re^h$ which we subindex as $z_{i,k}$ with $k=n+1\ldots m-1$. Express the output $y_i$, $i=1\ldots n$
\begin{equation}
    y_i = \alpha_{i,0}+\sum_{k=1}^n \alpha_{i,k} x_k+ \sum_{l=n+1}^{m-1} \alpha_{i,l} z_{i,l}
\end{equation} This is just a linear combination of a fully connected hidden-output layer with linear output activation.  Node $z_{i,l}$ is simply a product of inputs of the form 
\begin{equation}
    z_{i,l} = \prod_{k=1}^n x_k^{d_{k,i,l}}\;\;\sum_k d_{k,i,l} \leq d
\end{equation}
This is a multiplicative node that connects to the input each input node $x_i$ with $d_i$ replicated edges and unit weight.

\begin{theorem}
  The polynomial $f(x;\alpha)$ and the continuous-time neural network $f_{NN}(x;w(\alpha))$ are exactly equal.
\end{theorem}
  

One issue that emerges is that Poly-Nets are continuous-time networks. Computational implementations may require  a switch to using additional numerical ordinary differential equation solvers. In the next section, we show examples of popular ode solvers expressible as neural networks so that a discrete-time neural network exactly equal to discretized polynomial dynamics can be easily constructed.


\texttt{(what does it mean by k-sparse? Neither Barron, 1993 nor Andoni, 2014 seems to give a definition about this. Does it mean the total number of monomials are $O(k)$?)}
